Multi-vehicle Dynamic Water Surface Monitoring

Repeated exploration of a water surface to detect objects of interest and their subsequent monitoring is important in search-and-rescue or ocean clean-up operations. Since the location of any detected object is dynamic, we propose to address the combined surface exploration and monitoring of the detected objects by modeling spatio-temporal reward states and coordinating a team of vehicles to collect the rewards. The model characterizes the dynamics of the water surface and enables the planner to predict future system states. The state reward value relevant to the particular water surface cell increases over time and is nullified by being in a sensor range of a vehicle. Thus, the proposed multi-vehicle planning approach is to minimize the collective value of the dynamic model reward states. The purpose is to address vehicles' motion constraints by using model predictive control on receding horizon, thus fully exploiting the utilized vehicles' motion capabilities. Based on the evaluation results, the approach indicates improvement in a solution to the kinematic orienteering problem and the team orienteering problem in the monitoring task compared to the existing solutions. The proposed approach has been experimentally verified, supporting its feasibility in real-world monitoring tasks.

==> src/bup.tex <==
\begin{figure}[htbp]\centering
   \subfloat[Butterworth function\label{fig:butter}]{\includegraphics[width=.50\columnwidth]{fig/fig_butter.pdf}}
   \subfloat[Sensor range model\label{fig:visibility}]{\includegraphics[width=.50\columnwidth]{fig/fig_butter_heatmap_cone.pdf}}
   \caption{The Butterworth function $f_b(x)$ \textbf{(a)} of varying degree $n_b$. The cut-off range is $c_b = 1$ in both figures and is denoted by red vertical dashed line. By inputting Euclidean distance, we model the sensor range as a function of two variables $f_{b2}(x,y)$ \textbf{(b)}. The function degree in second figure is $n_b = 8$.}
\label{fig:butterworth}
\end{figure}



\begin{figure}[h]\centering
\label{fig:butter}\includegraphics[width=\columnwidth]{fig/fig_butter.pdf}
   \caption{Plot of the Butterworth function in~\cref{eq:butter} of varying degree $n_b$. The cut-off range is $c_b = 1$ in both figures and is denoted by red vertical dashed line.}
\label{fig:butterworth_plot}
\end{figure}

\begin{figure}[h]\centering
\label{fig:visibility}\includegraphics[width=\columnwidth]{fig/fig_butter_heatmap_cone.pdf}
   \caption{Plot of the function in~\cref{eq:butter2} of degree $n_b = 8$ and cut-off range is $c_b = 1$. By inputting Euclidean distance of a vehicle from target, we model the sensor range.}
\label{fig:butterworth_3d}
\end{figure}


==> src/removed.tex <==
% Filename: removed.tex
% Date:     2022/11/13 12:26
% Author:   Jan Faigl

% - abstract.tex --------------------------------------------------------------
V4:

%The state reward value relevant to the particular water surface cell increases over time and is nullified by being in a vehicle's sensor range.

V3:
Repeated exploration of a water surface to detect objects of interest and their subsequent monitoring is important in search-and-rescue or ocean clean-up operations.
Since the location of any detected object is dynamic, we propose to address the combined surface exploration and monitoring of the detected objects by modeling spatio-temporal reward states and coordinating a team of vehicles to collect the rewards.
The model characterizes the dynamics of the water surface and enables the planner to predict future system states.
The state reward value relevant to the particular water surface cell increases over time and is nullified by being in a sensor range of a vehicle.
Thus, the proposed multi-vehicle planning approach is to minimize the collective value of the dynamic model reward states.
The purpose is to address vehicles' motion constraints by using model predictive control on receding horizon, thus fully exploiting the utilized vehicles' motion capabilities.
Based on the evaluation results, the approach indicates improvement in a solution to the kinematic orienteering problem and the team orienteering problem in the monitoring task compared to the existing solutions.
The proposed approach has been experimentally verified, supporting its feasibility in real-world monitoring tasks.

V2:

We study combined water surface exploration and object monitoring tasks utilizing centralized multi-agent planner.
Repeated exploration of a water surface for purpose of object detection and subsequent monitoring of such objects are important aspects of search-and-rescue or ocean clean-up operations.
As the positions of detected objects on water surface are dynamic, we propose to address the problem by modeling of spatio-temporal reward states in the area of interest and coordinating vehicles for the purpose of reward collection.
Our proposed approach outperforms state of the art planning methods in the studied task by modeling potential information gain and target movement as reward states of a non-linear dynamical model, addressing dynamics of the water surface by enabling planner to predict future system states.
Values of the rewards states increase in time and are nullified by state location being in a sensor range of a vehicle.
The multi-vehicle planning task is to minimize collective value of the model reward states; however, the planning needs to address the motion constraints of the vehicles.
Therefore, we propose to address the problem as a model predictive control on the receding horizon.
Simulation results indicate improvement over state of the art in kinematic orienteering problem and stability in closed-loop operation, proposed approach was experimentally verified in a real-world monitoring task.

\iffalse
The studied dynamic water surface monitoring combines area exploration, monitoring, and object detection tasks in a single problem formulation of modeling a spatio-temporal reward in the environment with a centralized multi-agent planner.
We propose to address the problem using a dynamical nonlinear reward model for real-time exploration and monitoring of detected objects.
States of the reward model represent expected information gain at discrete locations of the monitored area.
The reward generally increases in time and is nullified by the presence of an agent in the neighborhood of the particular location.
Besides, objects detected during monitoring modify reward to gain, and thus the expected collective agent behavior is to prioritize certain locations.
The multi-vehicle planning task is to minimize the reward held in the model; however, the planning needs to address the motion constraints of the vehicles.
Therefore, we propose to address the problem as a model predictive control on the receding horizon.
Since the exploration and monitoring are assumed to be on an infinite horizon, the finite horizon solution is periodically re-planned.
The proposed method has been deployed on unmanned aerial vehicles and experimentally verified in real-world monitoring tasks.
\fi

V1:

Area exploration, monitoring and object detection tasks have both recently been tackled by use of multi-robot systems.
Use of Unmanned Aerial Vehicles aided by vision capabilities is especially frequent.
This enables to utilize on-board vision sensors for information gathering tasks.
Exploration of an unknown environment and subsequent monitoring based on environment model are distinct tasks.
We formulate these as a single task by modeling a spatio-temporal reward in the environment with centralized multi-agent planner.
We propose a dynamical nonlinear reward model for real-time exploration and monitoring detected objects.
States of the reward model represent potential information gains at discrete points in space, which increase in time.
Presence of an agent in the neighborhood of position nullifies the reward in its state, modeling information collection.
Agents are represented as unmanned aerial vehicles, subject to constrains limiting their modeled dynamics.
The multi-vehicle planning task is to minimize reward held in the model and is formulated as a model predictive control on receding horizon.
Objects detected during monitoring modify reward gain, influencing collective agent behavior to prioritize monitoring of certain positions.
As the exploration and monitoring are assumed to be on infinite horizon, the finite horizon solution is periodically re-planned.
The formulation is implemented for use with Robot Operating System and experimentally tested in real-world monitoring task.


% - introduction.tex ----------------------------------------------------------
V4:

   %\item Solution of the introduced IMP-DR problem using MPC-based planning on receding horizon with a dynamic environment and vehicle models, enabling prediction of the future state of the dynamic environment.

V3:
In addition to the constrained information gain by the limited sensor range, the movement planning needs to consider vehicle motion constraints.
%Besides, the information gain is constrained by limited vehicle sensor range, and movement planning needs to consider vehicle motion constraints.


V2:

\IEEEPARstart{I}{n} this letter, we present a novel formulation of model-based multi-vehicle planning, denoted \emph{Incremental Motion Planning with Dynamic Reward} (IMP-DR), to address continual exploration and monitoring of water surface with objects of interest using dynamic spatio-temporal reward model.
The studied problem belongs to a class of monitoring scenarios in which, on encountering an object of interest during exploration, further monitoring for changes in state or location is needed.
Besides, it is also required to search the environment repeatedly, as new objects might become detectable in time.

The motivational scenario is to employ a fleet of \emph{Unmanned Aerial Vehicles}~(UAVs) in top-down visual monitoring of large water surfaces surrounding a central ship, where the water surfaces might not be static due to weather conditions.
The problem is related to informative motion planning to maximize information gathering along the planned trajectory~\cite{hollinger14ijrr} and the kinematic \emph{Orienteering Problem} (OP) \cite{Meyer2022} to find constrained reward-collecting trajectory for the vehicle.
We model the information to be gained from exploration and monitoring as dynamic reward states, whose position in the environment can change.
Hence, the underlying spatio-temporal reward model dynamics influence the expected information gain and we formulate the combined information collecting task as maximizing the collected reward on a receding horizon, i.e. minimizing weighted sum of the reward states.
While value of a reward states steadily increases in time, it is nullified by presence of reward state in sensor range of a vehicle.
The information gain is constrained by limited vehicle sensor range, and movement planning needs to consider the dynamic vehicle model constraints.

\begin{figure}[tb]
   \includegraphics[width=\columnwidth]{fig/uav_water_2.jpg}
   \caption{Experimental UAV performing water surface monitoring mission.\label{fig:uav_over_water}}
\end{figure}

We propose to address the studied problem using the \emph{Model Predictive Control} (MPC) approach that allows us to consider dynamical models of the vehicles, reward state dynamics and positions of objects being monitored.
The continuous dynamical models enable prediction of future environment and vehicle states, with computational complexity exponentially increasing with prediction horizon length.
Thus, information-gathering trajectories are computed on a limited control horizon, and closed-loop operation scheme of the MPC planner enables continual exploration and monitoring with multiple vehicles.
A top-down snapshot from performed experimental monitoring deployment can be seen in Fig.~\ref{fig:plan_example}, where values of the reward states are overlaid.
%JF: every figure needs to be referenced.

\begin{figure}[tb]
   \includegraphics[width=\columnwidth]{fig/overlay_145.pdf}
   \caption{Reward value overlay during monitoring experiment using 2 UAVs.
   \label{fig:plan_example}}
\end{figure}

The main contributions are considered as follows.
\begin{itemize}
   \item Novel IMP-DR problem formulation to coordinate a team of vehicles to search a priory unknown water surface and monitor detected dynamic objects continually.
   \item Solution of the introduced IMP-DR problem using MPC-based planning on receding horizon which utilizes dynamic environment and vehicle models, enabling prediction of future environment state to address the dynamic water surface environment.
   \item Evaluation of the proposed solution and comparison with the most related (to the best of authors' knowledge) approach to the \emph{Team Orienteering Problem} (TOP)~\cite{chao1996team} adapted for the receding horizon planning with dynamic model and solved by the state-of-the-art meta-heuristic~\cite{pedersen2021grasp}.
     Proposed approach is also compared to the state-of-the-art kinematic OP methods~\cite{Meyer2022} for single vehicle, which it is shown to outperform in provided data.
   \item Experimental deployment of the proposed approach in real-world flight in a water surface monitoring scenario.
\end{itemize}

The remainder of the letter is organized as follows.
An overview of related work is provided in the following section.
The addressed problem is formally introduced as the IMP-DR in \cref{sec:problem}.
The used sensor and reward models are described in \cref{sec:models} together with the vehicle model and its motion constraints.
The proposed MPC-based solution is presented in \cref{sec:mpc}. 
Evaluation results and experimental deployment are reported in~\cref{sec:results}.
Concluding remarks are detailed in~\cref{sec:conclusion}.



   %\vspace*{-2em}
   %\vspace{-2em}

   %\begin{figure}[htb]
%   \includegraphics[width=\columnwidth]{fig/heatplot_10.pdf}
   %\vspace*{-2em}
%   \caption{Heat-map of reward with two monitoring UAV trajectories in their respective colors during experimental evaluation. \label{fig:two_map_small}}
   %\vspace{-2em}
%\end{figure}

V1:
Teams of both homogenous and heterogenous robots have recently been employed in monitoring tasks and enable efficient information gathering in scenarios where only manned presence would be difficult or dangerous.
Specifically search and rescue operations and disaster response frequently require monitoring over large areas.
On encountering an object of interest or some anomaly, we seek to monitor it further for changes an state or position.
It is also required to search the environment repeatedly, as new objects might become detectable in time.
By modeling the information gain from both exploration and monitoring as dynamically evolving reward, we can formulate the monitoring task as maximization of collected reward on a receding horizon.
The proposed IMP-DR formulation is based on the Incremental Informative Motion Planning presented in~\cite{sampling_based}.

We are motivated by top-down visual monitoring of a large water surface surrounding a central ship, serving as a base of operations for a fleet of~\emph{Unmanned Aerial Vehicles}~(UAVs).
The UAVs have to be coordinated in an efficient manner to continuously search surrounding area and monitor eventually detected anomalies at the same time.
The detected anomalies might be moving, as water surfaces are not static due to weather conditions which we assume to be known.
The vehicle movement is governed by dynamic models subject to constraints, the information gain by sensors model with limited range.
This introduces need to model the vehicles, sensors, environment and information held in it and to utilize a model-based planner.
We propose a planning method based on \emph{Model Predictive Control}~(MPC) to utilize these dynamic models. 
Information gathering solutions are computed on a planning horizon, and a closed-loop operation scheme addresses the continuous exploration and monitoring tasks with multiple vehicles.

Unlike informative planning formulations which utilize Gaussian regression to create a model of environment using collected information, we model the spatio-temporal information in the environment, vehicle sensors and vehicle dynamics as a set of continuous \emph{Ordinary Differential Equations} (ODEs).
A solution which utilizes vehicles to collect reward, representing the information, is provided by a \emph{Model Predictive Control}~(MPC) solver.
Reward model states correspond to positions in the environment where information can be gained.
Reward positions lie in a two dimensional space, and can also exhibit continuous dynamics.
Additional states represent dynamics of the vehicles, positions and velocities in both axes.
System inputs are accelerations of the vehicles.
Vehicle dynamics are subject to constraints, limiting maximum magnitude of velocity vector and maximum acceleration in each axis.
The vehicle constraints are modeled to address limitations of utilized multi-rotor UAV trajectory tracker.
Values of the reward model states increase in time, therefore, there is always reward to be collected, formulating the monitoring task.
We take advantage of dynamics of these models, as the model is evolving on each MPC sampling step, to formulate spatio-temporally aware planning.
Presence of an agent in neighborhood of some position nullifies the corresponding reward state, which corresponds to collection of the reward.
This is done by utilizing the Butterworth function-based reward collection model of vehicle sensor.
With large sensor ranges, vehicle can collect reward from multiple states at the same time with collection rate dependent on distance.
Reward state values can also be interpreted as time since last agent was present in the state neighborhood.
On detection of object to be more closely monitored, its position can be added as an additional reward state.
The MPC solver is utilized to provide solutions and the planning is performed on receding horizon with a fixed re-planning rate in closed-loop operation.


The proposed models and control scheme were implemented in the Python programming language using the do-mpc toolbox~\cite{dompc}, utilizing the Ipopt~\cite{ipopt} non-linear optimization framework.
Several sparse symmetric indefinite linear solver for the Ipopt were benchmarked to choose the best performing one for further evaluation of the proposed approach.
Model and planner were adapted for use with \emph{Robot Operating System}~(ROS) control pipeline making use of MRS UAV System~\cite{mrs_system} for simulation and experimental validation.

The main contributions of this paper are summarized below.
\begin{itemize}
   \item Novel Incremental Motion Planning with Dynamic reward is introduced to maximize information gain on limited time horizon by utilizing information model, sensor model and constrained vehicle model.
   \item The planning is formulated as a MPC task on receding horizon for continual exploration and adaptive monitoring of water surface in closed-loop operation.
   \item The proposed solution approach is computationally evaluated and compared against state-of-the-art Team Orienteering Problem meta-heuristic adapted for receding horizon planning with dynamic model.
   \item We experimentally evaluate the proposed solution approach in real-world flight in a water surface monitoring scenario.
\end{itemize}

The remainder of the paper is organized as follows.
An overview of related work on is provided in the following section.
The addressed problem is defined in Section~\ref{sec:problem} to formalize the IMP-DR.
The sensor, reward and vehicle models are described in Section~\ref{sec:models}.
The MPC solution method is introduced in Section~\ref{sec:mpc}, implementation details and tuning parameters are documented.
Computational evaluation of the proposed solution method and experimental evaluation are presented in~\ref{sec:results}.
Concluding remarks are detailed in Section~\ref{sec:conclusion}.



% - related.tex ---------------------------------------------------------------
V4:
%TODO A distributed multi-vehicle information collection approach presented in~\cite{julian2012distributed} utilizes a Bayesian filter to infer the environment state and collectively maximize the informativeness of measurements.
%This minimizes uncertainty of measured environment state with vehicles' movement based on the utility gradient but does not predict future states of the environment.

%\reviewi{The dynamics of water surface debris is studied in~\cite{durgadoo2021strategies}, showing that additional effects along with the local oscillations should be accounted for.

%reviewii \cite{lan2014variational};  - mentioned
%reviewii \cite{julian2012distributed}; -- do not include
%reviewii \cite{smith2012persistent},  -- mentioned 
%reviewii \cite{yu2014correlated} -- mentioned

%, and trajectories using multiple interception vehicles.

V3:

Environment monitoring can be formulated as a problem of creating a quantifiable phenomena model using sampled data from the environment~\cite{adaptive_sampling} with the regression about the phenomena state using some regression models such as \emph{Gaussian Processes} (GPs)~\cite{tresp2000mixtures} and a sensor model such as in~\cite{tigris}.
However, the studied continual monitoring task has to address vehicle motion constraints and autonomous information dynamics.
Therefore, path planning is a part of the vehicle navigation towards the locations where the studied phenomena can be measured, such as the signal strength~\cite{adaptive_informative}.
Informative path planning~\cite{adaptive_selection} is then to find the most informative path improving the phenomena model with respect to motion constraints of information collecting vehicles~\cite{hollinger14ijrr,ghaffari2019sampling}.

The aforementioned planning approaches are suitable for modeling spatial phenomena in environment monitoring tasks, but they do not address the underlying temporal dynamics that we call information dynamics and its interaction with the vehicles.
\reviewii{These are addressed by the persistent multi-vehicle monitoring of a changing environment represented with limited vehicle sensing range in~\cite{smith2012persistent}.
The vehicles are assumed to be traveling on pre-determined closed paths with velocity as a control input.}
\reviewii{Authors of~\cite{lan2014variational} address continuous monitoring of a dynamic scalar field over arbitrarily long horizon, where individual filtered measurements are used for value estimation.
They utilize the Pontryagin's minimum principle in combination with a numeric solver for planning locally optimal, single-vehicle sensing trajectories minimizing the estimation uncertainty, and single-order integrator vehicle dynamics are considered with unconstrained input.
A distributed multi-vehicle information collection approach presented in~\cite{julian2012distributed} utilizes Bayesian filter to infer environment state and collectively maximize informativeness of measurements.
This minimizes uncertainty of measured environment state with vehicles' movement based on the utility gradient, but do not predict future states of the environment.}
In our addressed task, we explicitly model the environment information dynamics \reviewii{similarly to the accumulation function in~\cite{smith2012persistent} in combination with sensor and vehicle dynamics} as a set of \emph{Discrete Algebraic Equations} (DAEs) used for moving-horizon prediction and control.
The limited prediction horizon allows planning to visit only some locations to collect measurements.
Hence, we need to select the most informative locations reachable; the task is formulated as a generalization of the \emph{Orienteering Problem} (OP)~\cite{vansteenwegen_orienteering_2011}.


V2:

%JF: avoid recently, usually , especially frequent and any similarly vague terms

Environment monitoring tasks can be formulated as Informative Sampling or Adaptive Informative Sampling\cite{adaptive_sampling} to create an environment model from the sampled data.
Regression can be then based on \emph{Gaussian Processes} (GPs)~\cite{tresp2000mixtures}.
Planning is then employed in robot navigation towards the particular parts of the environment to measure the studied phenomena such as signal strength~\cite{adaptive_informative}.
Finding the most informative path with respect to the motion constraints given by vehicle kinematics is addressed as informative path planning~\cite{adaptive_selection}. 
It has been further generalized to consider sampling-based motion planning in continuous space in~\cite{hollinger14ijrr}.
These approaches, suitable for modeling of quantifiable environment phenomena, do not directly address underlying information and vehicle dynamics, which we model as a set of continuous \emph{Ordinary Differential Equations} (ODEs).

Having an explicitly limited travel budget that does not allow visiting all possible locations to collect measurements, the problem can be formulated as a variant of the \emph{Orienteering Problem} (OP).
Such formulations, while not addressing the information dynamics, can be readily utilized in receding horizon reward collection planning scheme.
The authors of~\cite{pedersen2021grasp} formulate multi-vehicle planning tasks for search and rescue operations with grid-sampled rewards determined by satellite imaging of the area of interest.
However, this requires vehicles to visit exact sampled grid positions, constraining movement to a graph.
Formulation in~\cite{penivcka2019data} addresses data collection with non-zero sensing range and Dubins vehicle dynamics, the~\cite{Meyer2022} presents time-optimal multi-rotor vehicle kinematic trajectory generation.
The problem with multiple Dubins vehicles with limited travel budget is studied in~\cite{zahradka2018route}. 
Flooded area exploration using multiple UAVs presented in~\cite{garg2022directed} addresses the information reward to be collected by uniform sampling of grid cells in the environment, and utilizes a reinforcement learning model to develop travel budget constrained vehicle-driving policy.
The vehicle sensor range and vehicle movement are limited to the individual grid cells, vehicle dynamics or sensor is not accounted for.

To address dynamic position of target objects, the authors of~\cite{khosravi2015maximum} formulate approach utilizing receding horizon planning and dynamic clustering to maximize reward collected from moving targets with uncertain dynamics and trajectories using multiple interception vehicles.
In~\cite{khosravi2016cooperative}, the approach is further generalized to address obstacles in the cooperative planning.
On the other hand, cooperative planning on receding horizon can be based on the Fisher information matrix model, used in multi-UAV target tracking~\cite{koohifar2017receding}.
These receding horizon formulations address dynamics of target positions and vehicles, but not of the reward values, therefore, are unsuitable for monitoring tasks.
The approach in~\cite{luo2017distributed} investigates coordination of multiple wheeled robots in multiple moving target interception based on combination of target-switching and Voronoi-based coverage control law.
Repeated interception of a target, therefore monitoring, isn't addressed.


\iffalse
\todo{JF: You do not provide any comments what are the drawbacks of the existing approaches and why they cannot be utilized}
\revise{
Unlike informative planning formulations which utilize Gaussian regression to create a model of environment using collected information, we model the spatio-temporal information in the environment, vehicle sensors and vehicle dynamics as a set of continuous \emph{Ordinary Differential Equations} (ODEs).
A solution which utilizes vehicles to collect reward, representing the information, is provided by a \emph{Model Predictive Control}~(MPC) solver.
Reward model states correspond to positions in the environment where information can be gained.
Reward positions lie in a two dimensional space, and can also exhibit continuous dynamics.
Additional states represent dynamics of the vehicles, positions and velocities in both axes.
System inputs are accelerations of the vehicles.
Vehicle dynamics are subject to constraints, limiting maximum magnitude of velocity vector and maximum acceleration in each axis.
The vehicle constraints are modeled to address limitations of utilized multi-rotor UAV trajectory tracker.
Values of the reward model states increase in time, therefore, there is always reward to be collected, formulating the monitoring task.
We take advantage of dynamics of these models, as the model is evolving on each MPC sampling step, to formulate spatio-temporally aware planning.
Presence of an agent in neighborhood of some position nullifies the corresponding reward state, which corresponds to collection of the reward.
This is done by utilizing the Butterworth function-based reward collection model of vehicle sensor.
With large sensor ranges, vehicle can collect reward from multiple states at the same time with collection rate dependent on distance.
Reward state values can also be interpreted as time since last agent was present in the state neighborhood.
On detection of object to be more closely monitored, its position can be added as an additional reward state.
The MPC solver is utilized to provide solutions and the planning is performed on receding horizon with a fixed re-planning rate in closed-loop operation.
}
\fi

V1:
Recently, environment monitoring tasks have been formulated as Informative Sampling or Adaptive Informative Sampling\cite{adaptive_sampling}.
These are based on data sampling from the environment for the purpose of creation of environment models and make use of the~\emph{Gaussian Process} (GP) regressiong.
using for example create environment model for a regression such as using 
Some planning techniques are then used to navigate the robots, typically based on partitioning of the environment.
Such an approach is efficient when measuring some environment phenomena, e.g. WiFi signal strength~\cite{adaptive_informative}.
The Informative Path Planning~\cite{adaptive_selection} introduces limitations given by vehicle kinematics, the Incremental Informative Motion Planning~\cite{hollinger14ijrr} further introduces environment state estimation to limit possible vehicle trajectories and proposes receding horizon planning.

Reward collection in environment is often formulated as generalizations of the \emph{Orienteering Problem} (OP).
Dubins Team OP with Neighborhood~\cite{zahradka2018route} formalized collection of reward using multiple Dubins vehicles with limited travel budget.
Kinematic OP~\cite{Meyer2022} presents time-optimal multi-rotor and Dubins vehicle trajectory generation in data collection.
The Team OP solver presented in~\cite{pedersen2021grasp} formulates multi-vehicle planning task for search and rescue operations with grid-sampled rewards determined by satellite imaging of the area of interest.
In~\cite{penivcka2019data}, authors formulate the Dubins OP with Neighborhoods for data collection with non-zero sensing distance and Dubins vehicle dynamics.

The~\cite{khosravi2015maximum} presents formulation of the Maximum Reward Collection Problem with multiple vehicle in uncertain environments.
Receding-horizon planning and dynamic clustering is utilized to maximize reward collected from moving targets with uncertain dynamics.
It is further expanded upon in~\cite{khosravi2016cooperative} by addressing obstacles in the cooperative planner.
Cooperative planning on receding horizon in~\cite{koohifar2017receding} utilizes Fisher information matrix model for multi-UAV target tracking.

%JF: avoid recently, usually , especially frequent and any similarly vague terms

Environment monitoring tasks can be formulated as Informative Sampling or Adaptive Informative Sampling\cite{adaptive_sampling} to create an environment model from the sampled data.
Regression can be then based on \emph{Gaussian Processes} (GPs)~\cite{tresp2000mixtures}.
Planning is then employed in robot navigation towards the particular parts of the environment to measure the studied phenomena such as signal strength~\cite{adaptive_informative}.
Finding the most informative path with respect to the motion constraints given by vehicle kinematics is addressed as informative path planning~\cite{adaptive_selection}. 
It has been further generalized to consider sampling-based motion planning in continuous space in~\cite{hollinger14ijrr}.
These approaches, suitable for modeling of quantifiable environment phenomena, do not directly address underlying information and vehicle dynamics, which we model as a set of continuous \emph{Ordinary Differential Equations} (ODEs).

Having an explicitly limited travel budget that does not allow visiting all possible locations to collect measurements, the problem can be formulated as a variant of the \emph{Orienteering Problem} (OP).
Such formulations, while not addressing the information dynamics, can be readily utilized in receding horizon reward collection planning scheme.
The authors of~\cite{pedersen2021grasp} formulate multi-vehicle planning tasks for search and rescue operations with grid-sampled rewards determined by satellite imaging of the area of interest.
However, this requires vehicles to visit exact sampled grid positions, constraining movement to a graph.
Formulation in~\cite{penivcka2019data} addresses data collection with non-zero sensing range and Dubins vehicle dynamics, the~\cite{Meyer2022} presents time-optimal multi-rotor vehicle kinematic trajectory generation.
The problem with multiple Dubins vehicles with limited travel budget is studied in~\cite{zahradka2018route}. 
Flooded area exploration using multiple UAVs presented in~\cite{garg2022directed} addresses the information reward to be collected by uniform sampling of grid cells in the environment, and utilizes a reinforcement learning model to develop travel budget constrained vehicle-driving policy.
The vehicle sensor range and vehicle movement are limited to the individual grid cells, vehicle dynamics or sensor is not accounted for.

To address dynamic position of target objects, the authors of~\cite{khosravi2015maximum} formulate approach utilizing receding horizon planning and dynamic clustering to maximize reward collected from moving targets with uncertain dynamics and trajectories using multiple interception vehicles.
In~\cite{khosravi2016cooperative}, the approach is further generalized to address obstacles in the cooperative planning.
On the other hand, cooperative planning on receding horizon can be based on the Fisher information matrix model, used in multi-UAV target tracking~\cite{koohifar2017receding}.
These receding horizon formulations address dynamics of target positions and vehicles, but not of the reward values, therefore, are unsuitable for monitoring tasks.
The approach in~\cite{luo2017distributed} investigates coordination of multiple wheeled robots in multiple moving target interception based on combination of target-switching and Voronoi-based coverage control law.
Repeated interception of a target, therefore monitoring, isn't addressed.


\iffalse
\todo{JF: You do not provide any comments what are the drawbacks of the existing approaches and why they cannot be utilized}
\revise{
Unlike informative planning formulations which utilize Gaussian regression to create a model of environment using collected information, we model the spatio-temporal information in the environment, vehicle sensors and vehicle dynamics as a set of continuous \emph{Ordinary Differential Equations} (ODEs).
A solution which utilizes vehicles to collect reward, representing the information, is provided by a \emph{Model Predictive Control}~(MPC) solver.
Reward model states correspond to positions in the environment where information can be gained.
Reward positions lie in a two dimensional space, and can also exhibit continuous dynamics.
Additional states represent dynamics of the vehicles, positions and velocities in both axes.
System inputs are accelerations of the vehicles.
Vehicle dynamics are subject to constraints, limiting maximum magnitude of velocity vector and maximum acceleration in each axis.
The vehicle constraints are modeled to address limitations of utilized multi-rotor UAV trajectory tracker.
Values of the reward model states increase in time, therefore, there is always reward to be collected, formulating the monitoring task.
We take advantage of dynamics of these models, as the model is evolving on each MPC sampling step, to formulate spatio-temporally aware planning.
Presence of an agent in neighborhood of some position nullifies the corresponding reward state, which corresponds to collection of the reward.
This is done by utilizing the Butterworth function-based reward collection model of vehicle sensor.
With large sensor ranges, vehicle can collect reward from multiple states at the same time with collection rate dependent on distance.
Reward state values can also be interpreted as time since last agent was present in the state neighborhood.
On detection of object to be more closely monitored, its position can be added as an additional reward state.
The MPC solver is utilized to provide solutions and the planning is performed on receding horizon with a fixed re-planning rate in closed-loop operation.
}
\fi
These approaches, however, do not address continual monitoring tasks.

\revise{
Unlike informative planning formulations which utilize Gaussian regression to create a model of environment using collected information, we model the spatio-temporal information in the environment, vehicle sensors and vehicle dynamics as a set of continuous \emph{Ordinary Differential Equations} (ODEs).
A solution which utilizes vehicles to collect reward, representing the information, is provided by a \emph{Model Predictive Control}~(MPC) solver.
Reward model states correspond to positions in the environment where information can be gained.
Reward positions lie in a two dimensional space, and can also exhibit continuous dynamics.
Additional states represent dynamics of the vehicles, positions and velocities in both axes.
System inputs are accelerations of the vehicles.
Vehicle dynamics are subject to constraints, limiting maximum magnitude of velocity vector and maximum acceleration in each axis.
The vehicle constraints are modeled to address limitations of utilized multi-rotor UAV trajectory tracker.
Values of the reward model states increase in time, therefore, there is always reward to be collected, formulating the monitoring task.
We take advantage of dynamics of these models, as the model is evolving on each MPC sampling step, to formulate spatio-temporally aware planning.
Presence of an agent in neighborhood of some position nullifies the corresponding reward state, which corresponds to collection of the reward.
This is done by utilizing the Butterworth function-based reward collection model of vehicle sensor.
With large sensor ranges, vehicle can collect reward from multiple states at the same time with collection rate dependent on distance.
Reward state values can also be interpreted as time since last agent was present in the state neighborhood.
On detection of object to be more closely monitored, its position can be added as an additional reward state.
The MPC solver is utilized to provide solutions and the planning is performed on receding horizon with a fixed re-planning rate in closed-loop operation.
}

% - problem.tex ---------------------------------------------------------------
V2:

The \emph{Incremental Motion Planning with Dynamic Reward} (IMP-DR) problem is formulated as a multi-vehicle scenario considered in a two-dimensional environment represented by $n_p$ sampled locations or predicted positions of objects of interest, further referred to as targets, each encoded by a position vector $\matr{p}_i$.
Each $\matr{p}_i$ represents two coordinates $\matr{p}_i = \left[p_{i,x},\, p_{i,x}\right]$ and the targets form a discrete finite set $\mathcal{P} = \{ \matr{p}_i \in \real^2 : 1 \leq i \leq n_p \}$.
The number of targets $n_p$ can evolve during the mission as new targets might be added by the object detection pipeline.
\reviewi{Targets' position can change with predictable dynamics, model of which is assumed to be known.
Its' parameters however, might change during the monitoring based on visual observations.}
Thus, the target set is a function of time $\mathcal{P}(t)$ in the planning problem.

The presence of $m$ vehicles is assumed at the positions $\matr{q}_i = \left[q_{i,x},\,q_{i,x}\right]$ forming the set $\mathcal{Q} = \{ \matr{q}_i \in \real^2 : 1 \leq i \leq m  \}$.
The vehicles' positions change in time and can be explicitly denoted as $\mathcal{Q}(t)$.
The vehicles are subject to dynamical constraints given by the maximum velocity magnitude $\Vmax$ and acceleration in the axes $\Amax$.
Mutual vehicle collision avoidance and safety are addressed by the constraint on the minimum allowed distance between the vehicles $\Dmin$ at any time event $t$ such that $\norm{\matr{q}_i(t) - \matr{q}_j(t)} \geq \Dmin, \quad \forall \matr{q}_i(t), \matr{q}_j(t) \in \mathcal{Q}(t), i \neq j$, and $i,j\in\{1,\ldots, m\}$.

We seek to minimize the time elapsed between visits to the targets in $\mathcal{P}_t$ on a planning horizon $T_h$ while penalizing maximal value.
It is addressed by defining the dynamical reward state, analogous to the information in the informative planning approaches.
The reward states $r_i(t) \in \real^{+}_{0} : 0 \leq i \leq n_p$ are modeled for each $\matr{p}_i\in\mathcal{P}(t)$.
In the presence of any of the vehicles near the reward state position $\matr{p}_i$, its reward value $r_i$ is nullified.
Squared reward state value is used in optimization problems to penalize high values and improve solver performance.
The function $f_r(\dot{r},r,\mathcal{P},\mathcal{Q})$ describes implicit reward dynamics with relation to the targets and positions of the vehicles.
The variables of $f_r$ are functions of time; the notation is omitted for clarity.
We formulate the IMP-DR planning problem step as follows:

\vspace{-0.75em}   
\begin{equation}\label{eq:impdr}
  \begin{aligned}
    \optmin_{\mathcal{Q}} & = \sum_{i=1}^{n_p} \int_{t_0}^{T_0 + T_h} r_i^2 dt \\
    \text{s.t.   } \\
     & 0 = f_r(\dot{r},r,\mathcal{P},\mathcal{Q}).
  \end{aligned}
\end{equation}
\vspace{-0.75em}   

We utilize the IMP-DR to perform monitoring tasks by iterative solution of~\cref{eq:impdr}, incrementing the initial time $t_0$ with the sampling period $T_s \leq T_h$ on each iteration and utilizing the current reward state feedback.



V1:

\section{Problem Statement}\label{sec:problem}
The IMP-DR planning problem is formally described in this section.

A multi-vehicle scenario is considered in a two-dimensional environment, represented by $n_p$ sampled points of interest.
Each point position vector $\matr{p}_i$ holds two coordinates $\matr{p}_i = \left[p_{x,i},\, p_{y,i}\right]$.
All environment points belong to a set $\mathcal{P} = \{ \matr{p}_i \in \real^2 : 1 \leq i \leq n_p \}$.
Presence of $m$ vehicles is assumed at position vectors $\matr{q}_i = \left[q_{x,i},\,q_{y,i}\right]$.
All vehicle position vectors belong to a set $\mathcal{Q} = \{ \matr{q}_i \in \real^2 : 1 \leq i \leq m  \}$.
Vehicle are subject to dynamical constraints given by maximum velocity magnitude $\Vmax$ and acceleration in axes $\Amax$.
Vehicle collision avoidance is addressed by minimum allowed vehicle distance $\Dmin$, where $\norm{\matr{q}_i - \matr{q}_j} \geq \Dmin \quad \forall \matr{q}_i, \matr{q}_j \in \mathcal{Q}, i \neq j$.
Following established notation, the planning problems are described below as variations of problems presented in~\cite{hollinger14ijrr}.

We seek to minimize weighted time elapsed between visits to sampled points which are not static and can also be found during exploration.
Reward $r_i \in \real^{+}_{0} : 0 \leq i \leq n_p$ is given for each position and is part of the current environment state vector $\matr{s}$.
Positions of reward states are time dependent with known dynamics and also contained in $\matr{s}$.
Given $\matr{s} = \matr{s}_{t} \in \mathcal{S}$ as current environment state at the time $t$, function $f_s(\dot{s}_t,s_t,\mathcal{P}_t)$ describing the implicit environment dynamics, function $f_r(s_t,\mathcal{P})$ quantifying reward gain, $\mathcal{A}_t$ set of all possible collision-free UAV trajectories $\mathcal{P}_{i,t} \in \mathcal{P}_t$ up to time $t$ and $T$ as a planning horizon, we formulate the IMP-DR in~\cref{eq:impdr} planning problem as follows:

\begin{equation}\label{eq:impdr}
  \begin{aligned}
    \mathcal{P}^\ast_t & = \argmax_{\mathcal{P}_{t} \in \mathcal{A}_{t}} f_{t}(s_t,\mathcal{P}_{t}) \quad \forall t_s < t \leq T \\
    &\text{s.t.   } 0 = f_d(\dot{s}_t,s_t,\mathcal{P}_t)
  \end{aligned}
\end{equation}
% - method.tex ----------------------------------------------------------------

% - models.tex ----------------------------------------------------------------
V4:

% Dynamic: in motion, changing
% Dynamical: resulting from motion, e.g., friction or constraints

%TODO check the notation: Discrete vehicle positions $p_{x,i,k},p_{y,i,k}$ at sampled time-steps $k$ are used as the inputs of an indicator function to determine if a vehicle passed through the reward-collecting range during continual monitoring:

%TODO chec the notation: & \text{where}\ d_{i,j} = \sqrt{(p_{x,i} - q_{x,j,k})^2 + (p_{y,i} - q_{y,j,k})^2}.\nonumber





V3:
\subsection{Vehicle model}

\vspace{-2em}
\begin{multicols}{2}\noindent
   \begin{subequations}\label{eq:multi_rotor}
      \begin{align}
	 &\dot{q}_{x,i} = v_{x,i}T_s + a_{x,i}\frac{T_s^2}{2}\label{eq:multi_rotora}\\
	 &\dot{q}_{y,i} = v_{y,i}T_s + a_{y,i}\frac{T_s^2}{2}\label{eq:multi_rotorb}\\
	 &\dot{v}_{x,i} = a_{x,i}T_s\label{eq:multi_rotorc}\\
	 &\dot{v}_{y,i} = a_{y,i}T_s\label{eq:multi_rotord}\\
	 &~~~\text{for } 1 \leq i \leq m.\nonumber
      \end{align}
   \end{subequations}
   \begin{subequations}\label{eq:multi_rotor_con}
      \begin{align}
	 & \sqrt{v_{x,i}^2 + v_{y,i}^2} \leq \Vmax\label{eq:multi_rotor_cona}\\
	 & -\Amax \leq a_{x,i} \leq \Amax\label{eq:multi_rotor_conb}\\
	 & -\Amax \leq a_{y,i} \leq \Amax\label{eq:multi_rotor_conc}\\
	 &~~~\text{for } 1 \leq i \leq m.\nonumber
      \end{align}
   \end{subequations}
\end{multicols}
\vspace{-1em}

Collision avoidance puts minimal mutual distance constraints on the agents:
\vspace{-0.5em}
\begin{subequations}\label{eq:min_dist}
   \begin{align}
      &d_{i,j} \geq \Dmin, \\
      &d_{i,j} = \sqrt{(q_{x,i}-q_{x,j})^2 + (q_{y,i}-q_{y,j})^2},\\
      &~~~~~~\text{for } 1 \leq i,j \leq m,\ i \neq j.\nonumber
   \end{align}
\end{subequations}

\subsection{Water surface model}

\reviewi{The static water surface area is modeled as a finite grid of target points.

Movement of dynamic debris on the water is modeled as local periodic oscillations combined with a time-dependent drift, which is the simplified combined influence of water currents, sail effect and Stokes drift.
Precise modeling of underlying causes might improve the movement prediction, but is out of scope of this letter.
This is expressed for each axis as a simplified time-dependent function~\cref{eq:stokes} parameterized by amplitude $A_{\text{s}}$, angular velocity $\omega_{\text{s}}$ and the drift velocity $v_{\text{d}}$.
\begin{equation}\label{eq:stokes}
  x_{\text{s}}(t) = t v_{\text{d}} + A_{\text{s}}\sin{(t \omega_{\text{s}})}
\end{equation}
Parameters of this function are assumed to be known, but might vary during the monitoring for each target.
Change in the parameters could be then determined from visual measurements for adaptive monitoring.}

% - mpc.tex -------------------------------------------------------------------
Using the notation from~\cref{sec:problem} and models from~\cref{sec:models}, 


% - results.tex ---------------------------------------------------------------
V2:

%In particular, the performance of the proposed model-based planning approach is compared to the state-of-the-art Kinematic OP planner~\cite{Meyer2022} and Team OP meta-heuristic planner~\cite{pedersen2021grasp} with the results reported in \cref{sec:kinematicop} and \cref{sec:top}, respectively.

%The evaluation was performed using \emph{Robot Operating System}~(ROS) control pipeline of the MRS~UAV~System~\cite{mrs_system} and the AMD Ryzen 4750U processor running at the base clock of \SI{1.7}{\giga\hertz} and accompanied with \SI{32}{\giga\byte} RAM.

%The default solution convergence tolerance of $10^{-8}$ was used as the stopping criterion during evaluation.


V1:
Computational, simulation and experimental results of the proposed planning approach are described in this section.
vehicle number and horizon length influence on computational performance.

%Evaluation was performed on machine with the AMD Ryzen 4750U 8-core processor with the base clock of \SI{1.7}{\giga\hertz} and \SI{32}{\giga\byte} of RAM.
%up to \SI{4.1}{\giga\hertz} GHz single-core performance) and 32GB of RAM.

The average value of system state reward in time $r_{\text{avg}}$ exhibits Lyapunov stability, as it does not diverge from the neighborhood of some equilibrium $r_{\text{eq}}$ in $t\to\infty$.

\iffalse
Influence of planning horizon length $N_s$ on computational performance is presented in~\cref{tbl:horizon} and plotted in~\cref{fig:horizon}.
While increasing the $N_s$ leads to approximately polynomial increase in average step time $t_{\text{avg}}$, it does not necessarily lead to improvement in measured average reward equilibrium $r_{\text{avg}}$ and maximal reward $r_{\text{max}}$ (lower is better).
\begin{figure}[htbp]\centering
   \includegraphics[width=\columnwidth]{fig/comparison_horizon.pdf}
   \caption{Plot of $t_{\text{avg}}$ of solutions with varying number of vehicles $m$ and horizon length $N_s$ on a $10\times10$ grid.}
\label{fig:horizon}
  %\vspace{-1em}
\end{figure}
\fi


computational evaluation between the IMP-DR and state-of-the-art kinematic OP approaches.
The $t_{\text{avg}}$ denotes average MPC solver computational time of an instance.

% $C_{\text{\text{max}}} = \SI{10}{s}$ \textbf{(a)} and $C_{\text{\text{max}}} = \SI{45}{s}$ \textbf{(b)}.

%The solver is based on the \emph{Greedy Random Adaptive Search Procedure} (GRASP) meta-heuristic and the authors of~\cite{pedersen2021grasp} claim it experimentally provides a good trade-off between the computational requirements and solution quality compared to the exact \emph{Mixed Integer Linear Programming} (MILP) solution.


purpose of object detection is addressed by uniformly sampling the environment space.
Targets were sampled on a 

The models information collection dependent on distance.

%\subfloat[t=120s]{\includegraphics[width=0.5]{fig/exploration_120.pdf}}
%\subfloat[t=140s]{\includegraphics[width=0.5]{fig/exploration_140.pdf}}
%\subfloat[t=160s]{\includegraphics[width=0.5]{fig/exploration_160.pdf}}
%\subfloat[t=180s]{\includegraphics[width=0.5]{fig/exploration_180.pdf}}

  Square colors show values of sampled grid point reward states, determined by respective color bars. 

%\subfloat[t=120s]{\includegraphics[scale=0.5]{fig/monitoring_120.pdf}}
  %\subfloat[t=140s]{\includegraphics[scale=0.5]{fig/monitoring_140.pdf}}
  %\subfloat[t=160s]{\includegraphics[scale=0.5]{fig/monitoring_160.pdf}}
  %\subfloat[t=180s]{\includegraphics[scale=0.5]{fig/monitoring_180.pdf}}

   red a paths in the past $\SI{10}{s}$ are shown in their respective colors.

is addressed as monitoring of targets with predictable movement dynamics.

%TODO explicitely mention that - Such a setup in field conditions with limited computational resources is demonstrated in experimental evaluation.

As the utilization of Wi-Fi connection introduced delays in communication due to limited network bandwidth 

To account for data transfer delays introduced in real-world setup, the planning rate was lowered to


==> src/top.tex <==
% - section -------------------------------------------------------------------
\section{Team Orienteering Problem}\label{sec:top}

dynamic team orienteering bla bla bla

%\begin{figure}\centering

%\subfloat[] {
%  \includegraphics[width=0.3\textwidth]{../fig/coverage_w10_h20_n1_invdiv.csv}}
%\subfloat[] {
%  \includegraphics[width=0.3\textwidth]{../fig/coverage_w10_h20_n2_invdiv.csv}}
%\subfloat[] {
%  \includegraphics[width=0.3\textwidth]{../fig/coverage_w10_h20_n3_invdiv.csv}}
%\caption{Reward in 10x10 grid with 2 UAVs on a normalized planning horizon of 20. Median reward is shown as a solid line, while individual rewards as dashed. Individual instances from left to right are with neighbour level set to 1, 2 and 3 respectively.}
%\end{figure}
  


==> tbl/performance_data.tex <==
49 & 1 & 0.95&5.75&38.49&210.0\\
                49 & 2 & 3.25&17.51&26.00&153.0\\
                49 & 3 & 5.07&22.74&18.90&99.5\\
                49 & 4 & 9.22&38.90&16.73&90.5\\
                \hline\rule{0pt}{2ex}
                64 & 1 & 1.16&8.52&43.66&225.0\\
                64 & 2 & 3.83&13.70&30.66&180.5\\
                64 & 3 & 7.34&33.29&26.97&166.0\\
                64 & 4 & 12.48&63.53&24.22&177.0\\
                \hline\rule{0pt}{2ex}
                81 & 1 & 1.35&7.94&56.59&229.0\\
                81 & 2 & 4.77&21.49&35.37&191.5&\\
                81 & 3 & 8.40&56.60&30.31&178.5\\
                81 & 4 & 12.57&59.33&25.73&158.5\\
                \hline\rule{0pt}{2ex}
                100 & 1 &1.66&94.11&68.25&310.0\\
                100 & 2 &5.57&22.23&44.63&178.5\\
                100 & 3 &9.91&47.32&34.87&243.5\\
                100 & 4 &17.11&118.72&28.72&192.5\\


==> tbl/result_data_automated.tex <==
25 & 1 & 0.07 & 1.0 & 26.8 & 115.9\\
25 & 2 & 0.17 & 1.7 & 23.8 & 109.9\\
25 & 3 & 0.5 & 4.6 & 17.9 & 97.3\\
25 & 4 & 0.6 & 6.4 & 20.2 & 100.6\\
25 & 5 & 1.1 & 9.5 & 18.0 & 91.3\\
25 & 6 & 2.09 & 14.9 & \mathbf{6.4} & \mathbf{49.7}\\
\hline
36 & 1 & 0.12 & 0.7 & 28.0 & 144.2\\
36 & 2 & 0.23 & 2.2 & 25.9 & 132.5\\
36 & 3 & 0.92 & 7.2 & 19.1 & 107.2\\
36 & 4 & 1.96 & 14.2 & 11.3 & 62.2\\
36 & 5 & 2.82 & 18.6 & \mathbf{11.1} & \mathbf{58.5}\\
36 & 6 & 2.36 & 16.6 & 13.6 & 77.6\\
\hline
49 & 1 & 0.13 & 1.0 & 47.4 & 177.6\\
49 & 2 & 0.62 & 29.4 & 22.7 & 99.9\\
49 & 3 & 1.42 & 10.7 & 20.5 & 109.8\\
49 & 4 & 2.52 & 20.9 & 16.4 & \mathbf{72.2}\\
49 & 5 & 3.62 & 29.8 & 17.2 & 105.6\\
49 & 6 & 3.44 & 25.4 & \mathbf{13.5} & 86.1\\
\hline
64 & 1 & 0.16 & 1.9 & 52.1 & 215.1\\
64 & 2 & 0.91 & 6.4 & 30.2 & 126.0\\
64 & 3 & 1.94 & 21.0 & 24.8 & 109.8\\
64 & 4 & 3.02 & 20.7 & 20.0 & 98.7\\
64 & 5 & 3.82 & 23.2 & 16.6 & 76.1\\
64 & 6 & 4.84 & 42.4 & \mathbf{15.8} & \mathbf{74.0}\\
\hline
81 & 1 & 0.25 & 1.6 & 51.5 & 247.1\\
81 & 2 & 1.21 & 7.0 & 36.7 & 179.2\\
81 & 3 & 2.65 & 26.6 & 26.4 & 106.2\\
81 & 4 & 3.82 & 29.0 & 28.8 & 148.0\\
81 & 5 & 4.5 & 42.9 & 20.8 & 124.3\\
81 & 6 & 6.27 & 36.9 & \mathbf{18.6} & \mathbf{95.0}\\
\hline
100 & 1 & 0.35 & 2.7 & 63.4 & 237.5\\
100 & 2 & 1.67 & 20.1 & 33.7 & 159.7\\
100 & 3 & 2.0 & 14.7 & 29.8 & 127.1\\
100 & 4 & 3.37 & 71.3 & 25.9 & 133.4\\
100 & 5 & 4.65 & 24.0 & 25.7 & 130.7\\
100 & 6 & 7.07& 77.2 & \mathbf{22.6} & \mathbf{118.4}


==> tbl/result_data_automated_discrete-rounded.tex <==
25 & 1 & 0.05 & 1.5 & 32.7 & 109.8\\
25 & 2 & 0.12 & 2.0 & 27.6 & 139.2\\
25 & 3 & 0.55 & 5.8 & 16.7 & 97.7\\
25 & 4 & 0.77 &8.9 & \mathbf{9.9} & \mathbf{56.2}\\
25 & 5 & 1.06 & 8.8 & 13.7 & 94.6\\
25 & 6 & 1.22 & 12.1 & 16.4 & 86.2\\
\hline\noalign{\smallskip}
36 & 1 & 0.10 & 1.2 & 32.6 & 125.2\\
36 & 2 & 0.27 & 1.8 & 21.6 & 95.3\\
36 & 3 & 0.87 & 8.8 & 18.7 & 106.7\\
36 & 4 & 1.49 & 12.8 & 16.9 & 102.4\\
36 & 5 & 1.62 & 18.0 & 19.0 & 95.9\\
36 & 6 & 2.71 & 56.9 & \mathbf{13.0} & \mathbf{87.5}\\
\hline\noalign{\smallskip}
49 & 1 & 0.18 & 5.8 & 31.3 & 125.0\\
49 & 2 & 0.49 & 4.3 & 32.3 & 143.5\\
49 & 3 & 1.42 & 19.9 & 18.3 & 80.6\\
49 & 4 & 1.63 & 21.1 & 25.5 & 98.5\\
49 & 5 & 3.30 & 18.3 & 14.4 & 94.6\\
49 & 6 & 3.53 & 33.0 & \mathbf{13.3} & \mathbf{70.0}\\
\hline\noalign{\smallskip}
64 & 1 & 0.18 & 6.3 & 42.4 & 205.7\\
64 & 2 & 0.75 & 13.8 & 33.9 & 151.8\\
64 & 3 & 1.48 & 9.0 & 26.8 & 140.7\\
64 & 4 & 3.06 & 17.6 & 18.9 & 108.3\\
64 & 5 & 3.42 & 26.6 & \mathbf{17.4} & 112.1\\
64 & 6 & 4.48 & 28.9 & 17.7 & \mathbf{94.8}\\
\hline\noalign{\smallskip}
81 & 1 & 0.20 & 1.3 & 59.0 & 224.5\\
81 & 2 & 1.24 & 6.8 & 32.0 & 125.9\\
81 & 3 & 2.48 & 14.4 & 24.6 & 115.6\\
81 & 4 & 3.59 & 21.6 & 24.5 & 123.2\\
81 & 5 & 4.41 & 111.6 & 20.6 & 122.0\\
81 & 6 & 5.91 & 32.8 & \mathbf{19.4} & \mathbf{95.4}\\
\hline\noalign{\smallskip}
100 & 1 & 0.43 & 20.9 & 55.2 & 279.9\\
100 & 2 & 1.50 & 8.9 & 33.4 & 149.0\\
100 & 3 & 1.85 & 26.9 & 28.1 & 164.1\\
100 & 4 & 2.67 & 28.5 & 28.2 & 118.9\\
100 & 5 & 4.16 & 31.8 & 24.5 & 136.5\\
100 & 6 & 7.07 & 77.3 & \mathbf{22.7} & \mathbf{118.4}


==> tbl/result_data_automated_discrete.tex <==
25 & 1 & 0.05 & 1.47 & 32.74 & 109.78\\
25 & 2 & 0.12 & 1.95 & 27.63 & 139.17\\
25 & 3 & 0.55 & 5.75 & 16.67 & 97.36\\
25 & 4 & 0.77 &8.86 & \mathbf{9.93} & \mathbf{56.20}\\
25 & 5 & 1.06 & 8.81 & 13.72 & 94.56\\
25 & 6 & 1.22 & 12.08 & 16.39 & 86.21\\
\hline\noalign{\smallskip}
36 & 1 & 0.10 & 1.15 & 32.64 & 125.17\\
36 & 2 & 0.27 & 1.81 & 21.55 & 95.26\\
36 & 3 & 0.87 & 8.80 & 18.73 & 106.69\\
36 & 4 & 1.49 & 12.78 & 16.87 & 102.36\\
36 & 5 & 1.62 & 17.97 & 18.99 & 95.86\\
36 & 6 & 2.71 & 56.87 & \mathbf{13.00} & \mathbf{87.50}\\
\hline\noalign{\smallskip}
49 & 1 & 0.18 & 5.79 & 31.25 & 125.0\\
49 & 2 & 0.49 & 4.29 & 32.28 & 143.49\\
49 & 3 & 1.42 & 19.88 & 18.28 & 80.59\\
49 & 4 & 1.63 & 21.06 & 25.54 & 98.47\\
49 & 5 & 3.30 & 18.31 & 14.44 & 94.60\\
49 & 6 & 3.53 & 33.0 & \mathbf{13.26} & \mathbf{70.00}\\
\hline\noalign{\smallskip}
64 & 1 & 0.18 & 6.31 & 42.40 & 205.66\\
64 & 2 & 0.75 & 13.76 & 33.85 & 151.75\\
64 & 3 & 1.48 & 8.98 & 26.79 & 140.70\\
64 & 4 & 3.06 & 17.56 & 18.90 & 108.32\\
64 & 5 & 3.42 & 26.58 & \mathbf{17.37} & 112.09\\
64 & 6 & 4.48 & 28.92 & 17.70 & \mathbf{94.80}\\
\hline\noalign{\smallskip}
81 & 1 & 0.20 & 1.32 & 59.01 & 224.50\\
81 & 2 & 1.24 & 6.78 & 32.04 & 125.88\\
81 & 3 & 2.48 & 14.35 & 24.60 & 115.60\\
81 & 4 & 3.59 & 21.63 & 24.50 & 123.20\\
81 & 5 & 4.41 & 111.57 & 20.62 & 122.00\\
81 & 6 & 5.91 & 32.81 & \mathbf{19.35} & \mathbf{95.39}\\
\hline\noalign{\smallskip}
100 & 1 & 0.43 & 20.85 & 55.15 & 279.75\\
100 & 2 & 1.50 & 8.87 & 33.35 & 148.99\\
100 & 3 & 1.85 & 26.79 & 28.15 & 164.10\\
100 & 4 & 2.67 & 28.51 & 28.21 & 118.87\\
100 & 5 & 4.16 & 31.83 & 24.49 & 136.52\\
100 & 6 & 7.07 & 77.25 & \mathbf{22.68} & \mathbf{118.44}


==> tbl/result_horizon_automated_discrete-rounded.tex <==
1 & 10 & 0.05 & 0.5 & 74.2 & 159.8\\
1 & 15 & 0.11 & 1.2 & 66.6 & 159.8\\
1 & 20 & 0.26 & 2.5 & 61.9 & 159.8\\
1 & 25 & 0.76 & 6.0 & 46.1 & 159.8\\
1 & 30 & 1.18 & 10.1 & 46.9 & 159.8\\
4 & 10 & 0.33 & 7.2 & 56.6 & 159.8\\
4 & 15 & 1.23 & 5.3 & 24.4 & 112.9\\
4 & 20 & 2.52 & 39.1 & 25.4 & 124.1\\
4 & 25 & 5.9 & 35.4 & 20.6 & 115.4\\
4 & 30 & 9.98 & 105.8 & 22.8 & 101.0\\
6 & 10 & 0.43 & 32.0 & 47.0 & 155.7\\
6 & 15 & 2.36 & 77.1 & 23.4 & 159.8\\
6 & 20 & 7.07 & 77.3 & 18.7 & 118.4\\
6 & 25 & 18.71 & 238.6 & 18.5 & 133.5\\
6 & 30 & 33.51 & 242.5 & 16.3 & 100.0


==> tbl/result_horizon_automated_discrete.tex <==
1 & 10 & 0.05 & 0.45 & 74.19 & 159.75\\
1 & 15 & 0.11 & 1.22 & 66.57 & 159.75\\
1 & 20 & 0.26 & 2.52 & 61.85 & 159.75\\
1 & 25 & 0.76 & 5.99 & 46.08 & 159.75\\
1 & 30 & 1.18 & 10.06 & 46.89 & 159.75\\
4 & 10 & 0.33 & 7.17 & 56.64 & 159.75\\
4 & 15 & 1.23 & 5.25 & 24.35 & 112.87\\
4 & 20 & 2.52 & 39.07 & 25.38 & 124.14\\
4 & 25 & 5.9 & 35.43 & 20.59 & 115.35\\
4 & 30 & 9.98 & 105.82 & 22.77 & 100.96\\
6 & 10 & 0.43 & 31.95 & 46.97 & 155.72\\
6 & 15 & 2.36 & 77.12 & 23.44 & 159.75\\
6 & 20 & 7.07 & 77.25 & 18.67 & 118.44\\
6 & 25 & 18.71 & 238.59 & 18.46 & 133.5\\
6 & 30 & 33.51 & 242.48 & 16.26 & 100.02\\


==> tbl/tbl_combined.tex <==
\begin{table}[htbp]\centering


  \subfloat[][]{\centering
   \begin{tabularx}{0.5\columnwidth}{
	       C
	       C
	       R
	       R
	       R
	       R
	       R
	       R
	    }
      \toprule
      m & N_s & t_{\text{avg}}\text{[\si{s}]} &t_{\text{max}} \text{[\si{s}]}&r_{\text{eq}}\text{[-]}& r_{\text{max}} \text{[-]}\rule{0pt}{2ex}\\
      \midrule
	    \input{tbl/result_horizon_automated.tex}
      \bottomrule
	 \end{tabularx}
   \caption{Computational results for $m$ vehicles and horizon~$N_s$}\label{tbl:horizon}
     }
   \subfloat[][]{\centering
   \caption{Results for the Kinematic Orienteering Problem}\label{tbl:kop}
   \begin{tabularx}{0.5\columnwidth}{
	 R
	 R
	 R
	 R
	 R
	 R
      }
      \toprule
      C_{\text{max}} \text{[s]}&\text{KOP-1} & \text{KOP-6}^{\text{lns}} & \text{MPC}_{\text{best}} & t_{\text{avg}} \text{[s]}\\
      \midrule
      10 & 95 & 80 & \mathbf{115} &1.7 \\
      15 & 180 & 165 & \mathbf{200}&2.8 \\
      20 & 250 & 250 & \mathbf{260}&8.7 \\
      25 & 325 & 330 & \mathbf{370}&11.4 \\
      30 & 390 & 390& \mathbf{450}&15.9 \\
      35 & 430 & 435 & \mathbf{450}&22.8 \\
      40 & \mathbf{450} & \mathbf{450} & \mathbf{450}&45.7\\
      \bottomrule
   \end{tabularx}
     }
   \subfloat[][]{\centering
   \caption{Computational results for $n_p$ targets and $m$ vehicles}\label{tbl:vehicles_width}
      \begin{tabularx}{0.5\columnwidth}{
	    C
	    C
	    R
	    R
	    R
	    R
	    R
	    R
	 }
        \toprule
        n_p & m & t_{\text{avg}}\text{[\si{s}]} &t_{\text{max}} \text{[\si{s}]}&r_{\text{eq}}\text{[-]}& r_{\text{max}} \text{[-]}\rule{0pt}{2ex}\\
        \midrule
	 \input{tbl/result_data_automated.tex}
        \bottomrule
      \end{tabularx}
     }
\end{table}

